Safety-Critical Edge Robotics Architecture with Bounded End-to-End Latency

Edge computing processes data near its source, reducing latency and enhancing security compared to traditional cloud computing while providing its benefits. This paper explores edge computing for migrating an existing safety-critical robotics use case from an onboard dedicated hardware solution. We propose an edge robotics architecture based on Linux, Docker containers, Kubernetes, and a local wireless area network based on the TTWiFi protocol. Inspired by previous work on real-time cloud, we complement the architecture with a resource management and orchestration layer to help Linux manage, and Kubernetes orchestrate the system-wide shared resources (e.g., caches, memory bandwidth, and network). Our architecture aims to ensure the fault-tolerant and predictable execution of robotic applications (e.g., path planning) on the edge while upper-bounding the end-to-end latency and ensuring the best possible quality of service without jeopardizing safety and security.

==> Makefile <==
paper=Main.pdf
bibs=References.bib
main=Main
codes=$(wildcard code/*/*.c)
srcs=$(wildcard *.tex) $(wildcard *.tex)
images=$(wildcard images/*.png) $(wildcard images/*.pdf) \
			 $(wildcard images/*/*.png) $(wildcard images/*/*.pdf)
figs=$(wildcard figures/*.tex)
figs_pdf=$(patsubst %.tex, %.pdf, $(figs))
figs_png=$(patsubst %.tex, %.png, $(figs))

pdf: $(paper)
	@echo "======================================================="
	@echo "== Generated document can be found in $(paper) =="
	@echo "======================================================="

figures: $(figs_pdf)

png: $(figs_png)
	@echo "==================================================="
	@echo "== Generated figures can be found in figures/png =="
	@echo "==================================================="

all: pdf png

$(paper): $(srcs) $(bibs) $(figs_pdf) $(codes) Makefile
	@ mkdir -p tmp/ && echo "Successfully created tmp/chapters folder"
	@printf "Creating $@ ...\n"
	@(latexmk -pdf -output-directory=tmp -pdflatex='pdflatex -synctex=1' -halt-on-error -quiet $(main).tex) 2> tmp/latexmk.log 1> tmp/latexmk.out || ( printf "... FAILED!!!! (check tmp/$(main).log for errors, specially the lasts lines)\n" && exit 1 )
	@mv tmp/$(main).pdf $@
	@mv tmp/$(main).synctex.gz $(main).synctex.gz
	@printf "...done\n"

figures/%.pdf: figures/%.tex Makefile 
	@mkdir -p tmp/$(basename $@) && printf "Successfully created tmp/$(basename $@) folder\n"
	@printf "Creating figure $@ ...\n"
	@(latexmk -pdf -output-directory=tmp/$(basename $@) -halt-on-error -quiet $<) 2> tmp/$(basename $@)/latexmk.log 1> tmp/$(basename $@)/latexmk.out || ( printf "... FAILED!!!! (check log in tmp/$(basename $@)/$(basename $(notdir $@)).log for errors, specially the lasts lines)\n" && exit 1 )
	@mv tmp/$(basename $@)/$(notdir $@) $(basename $@).pdf
	@printf "...done\n"

figures/png:
	mkdir -p figures/png

figures/%.png: figures/%.pdf figures/png
	convert -density 600 $< $@

distclean:
	rm -rf tmp $(paper) $(main).synctex.gz
	@for fig in $(figs_pdf) $(figs_png); do \
		if [ -e $${fig} ]; then\
			echo "rm -f $${fig}"; \
			rm -f $${fig}; \
		fi;\
	done

clean:
	rm -rf $(paper) figures/*.pdf $(main).synctex.gz

==> Section_How_To.tex <==
% !TEX root = Main.tex
%
% This section explains how to use this template to write the paper
\svnid{$Id: Section_How_To.tex 10 2024-04-09 09:19:02Z maia $}
%----------------------Do not modify above-------------------------
\section{How to Use Commenting in this Document}

This document supports commenting. The main styles for comments are included in "comment.tex" file. 
There are 6 types of comments:
\begin{itemize}
	\item \textbf{Main Comment}: Green comments are used to show main comment about some part of the text. 
	Name of the person appears in the beginning of the comment if that person is already defined in "comments.tex" file. 
	We usually use combination of the first name and last name. 
	For example, "gg" stands for Gautam Gala. 
	Thus, \textit{ggcomment} command appears with name "GG".
	Example: \gfcomment{Sample comment by Gerhard.}  \ggcomment{Sample comment by Gautam.} 
	
	\item \textbf{Anonymous Comment}: For anonymous comment, or for those who are not in the "comments.tex" file, it is possible to use \textit{comment} command. Example: \comment{Anonymous comment.}
	
	\item \textbf{Main Reply}: It is used to show that the following message is a reply to a comment. 
	Example: 
	\ggreply{Sample replay comment by Gautam. } 
	\\
	\reply{Anonymous reply.}
	
	\item \textbf{Figure is Missing Comment}: This comment shows a figure is missing. 
	Example: 
	\ggfiguremissing{Here we need Figure 2.}
	
	\item \textbf{Side Comment}: Side comments appear close to the text, and not as a part of text. For these comments, write as minimum words as possible. 
	They make the document ugly, but they are easy to trace. 
	Example: 
	\ggsidecomment{Test}
	\textbf{Note:} If you use this comment, you need to compile the document 3 times to get your correct comment right. ;-)
	
	\item \textbf{Outline Comment}: All previous comments are inline. 
	If you want to show itemized lists use outlines. 
	Outlines are not assigned to people's names. 
	Example:
	\outline{ Here we have an outline. 
	\begin{itemize}
		\item It can have several items.
		\item It accepts many types of formatting.
		\item It highlights the concerns.
		\item It is very useful for structuring the text. 
	\end{itemize}
	}
	\item Example figure and image
	\begin{figure}[h!bt]
		\centering
		%\includegraphics[width=.5\textwidth]{figures/RM_flat.pdf}
		\caption{example figure (tikz) }\label{fig:RM_flat}
	\end{figure}
	
	\begin{figure}[h!bt]
		\centering
		\includegraphics[width=.5\textwidth]{images/rts.jpg}
		\caption{example image}\label{fig:Rts}
	\end{figure}

\end{itemize}

















==> Section_PoC.tex <==
% !TEX root = Main.tex
%
% Existing use case
\svnid{$Id: Section_PoC.tex 7 2024-04-03 15:03:54Z gala $}
%----------------------Do not modify above-------------------------
\section{Proof-of-Concept Simulation}
\label{section:experiments}
\ggcomment{Estimated size: 0.5 column}
\incharge{IK}
\outline{
	do some proof of concept runs of robotic apps on the intel server with our Linux/LVM and show some initial results
}
